Do End-to-end Stereo Algorithms Under-utilize Information?

Deep networks for stereo matching typically leverage 2D or 3D convolutional encoder-decoder architectures to aggregate cost and regularize the cost volume for accurate disparity estimation. Due to content-insensitive convolutions and down-sampling and up-sampling operations, these cost aggregation mechanisms do not take full advantage of the information available in the images. Disparity maps suffer from over-smoothing near occlusion boundaries, and erroneous predictions in thin structures. In this paper, we show how deep adaptive filtering and differentiable semi-global aggregation can be integrated in existing 2D and 3D convolutional networks for end-to-end stereo matching, leading to improved accuracy. The improvements are due to utilizing RGB information from the images as a signal to dynamically guide the matching process, in addition to being the signal we attempt to match across the images. We show extensive experimental results on the KITTI 2015 and Virtual KITTI 2 datasets comparing four stereo networks (DispNetC, GCNet, PSMNet and GANet) after integrating four adaptive filters (segmentation-aware bilateral filtering, dynamic filtering networks, pixel adaptive convolution and semi-global aggregation) into their architectures. Our code is available at https://github.com/ccj5351/DAFStereoNets.

==> evaluation_vkt2.tex <==
% as a backup table: with sub-tables, (a) and (b). 
\begin{table*}[t]
\small
\centering
\scalebox{0.96}{
    %\begin{tabularx}{1.0\linewidth}{p{0.75cm} | XX XX XX XX}
    %\begin{tabularx}{1.0\linewidth}{@{} p{0.75cm} | YYY| YYY |YYY | YYY @{}}
    \begin{tabularx}{1.0\linewidth}{@{} ?{1pt} p{0.75cm} ?{1pt} YYY ?{1pt} YYY  ?{1pt}YYY ?{1pt} YYY ?{1pt} @{}}
    %\hline
    \Xhline{2\arrayrulewidth}
	\multirow{3}{0.8pt}{{\bf Filters}} & \multicolumn{3}{c ?{1pt} }{ \bf DispNetC} & \multicolumn{3}{c ?{1pt}  }{ \bf PSMNet}  & \multicolumn{3}{c ?{1pt}  }{ \bf GANet} & \multicolumn{3}{c ?{1pt}}{ \bf GCNet} \\
	\cline{2-13} % draw a horizontal line spanning only some of the table cells
	%&\multicolumn{8}{c}{Bad-3.0 Error Rates (\%)}  \\
	 &{EPE(px)}  &{$\geq 1$ px} &{$\geq 3$ px} &{EPE(px)}  &{$\geq 1$ px} &{$\geq 3$ px} &{EPE(px)}  &{$\geq 1$ px} &{$\geq 3$ px} &{EPE(px)}  &{$\geq 1$ px} &{$\geq 3$ px} \\
	%\hline \hline
	\Xhline{2\arrayrulewidth}
	W/O & 0.68 & 11.54 & 3.72  &0.45   & 7.08  & 2.21  & \textbf{0.33}  & \textbf{5.34} & \textbf{1.70}  & 0.62  & 9.71 & 3.18 \\
	%\hline
	\Xhline{2\arrayrulewidth}
	\cellcolor{myskyblue}SABF & \cellcolor{mygray}0.65 & \cellcolor{mygray} 10.86 & \cellcolor{mygray} 3.48  & \cellcolor{mygray}\textbf{0.36} & \cellcolor{mygray}\textbf{5.92} & \cellcolor{mygray}\textbf{1.98}  & 0.34 & 5.50 & 1.76  & \cellcolor{mygray}0.60 & 9.89  & 3.19  \\
	\cellcolor{myskyblue} DFN & \cellcolor{mygray} \textbf{0.57} & \cellcolor{mygray}9.85 & \cellcolor{mygray}3.26  & \cellcolor{mygray}0.42  & \cellcolor{mygray}6.45 & \cellcolor{mygray}2.17  & 0.37  & 6.23 & 1.99  & \cellcolor{mygray}0.60 & \cellcolor{mygray}9.20 & \cellcolor{mygray}3.11  \\
	\cellcolor{myskyblue}PAC & \cellcolor{mygray}0.58 & \cellcolor{mygray}9.92 & \cellcolor{mygray}3.39  & 0.52  & 7.81  & 2.61   & 0.40  & 7.01 & 2.20  & 0.75 & 12.98 & 4.02  \\
	\cellcolor{myskyblue}SGA & \cellcolor{mygray}\textbf{0.57} & \cellcolor{mygray}\textbf{9.37} & \cellcolor{mygray}\textbf{3.21} & \cellcolor{mygray}0.40 & \cellcolor{mygray}6.08 & \cellcolor{mygray}2.14  &- &- &-  & \cellcolor{mygray}\textbf{0.55} & \cellcolor{mygray}\textbf{9.24} & \cellcolor{mygray}\textbf{2.98}  \\
	%\hline
	\Xhline{2\arrayrulewidth}
	\end{tabularx}}

\vspace{-4pt}

\caption*{(a) Evaluation on VKT2 validation set of Scene01, 02, 18 and 20.
}
\label{tab:vkt2-val-wo-scene6}
\vspace{3pt}
\centering
\scalebox{0.96}{
    %\begin{tabularx}{1.0\linewidth}{p{0.75cm} | XX XX XX XX}
    %\begin{tabularx}{1.0\linewidth}{@{} p{0.75cm} | YYY| YYY |YYY | YYY @{}}
    \begin{tabularx}{1.0\linewidth}{@{} ?{1pt} p{0.75cm} ?{1pt} YYY ?{1pt} YYY  ?{1pt}YYY ?{1pt} YYY ?{1pt} @{}}
    %\hline
    \Xhline{2\arrayrulewidth}
	\multirow{3}{0.8pt}{{\bf Filters}} & \multicolumn{3}{c ?{1pt} }{ \bf DispNetC} & \multicolumn{3}{c ?{1pt}  }{ \bf PSMNet}  & \multicolumn{3}{c ?{1pt}  }{ \bf GANet} & \multicolumn{3}{c ?{1pt}}{ \bf GCNet} \\
	\cline{2-13} % draw a horizontal line spanning only some of the table cells
	%&\multicolumn{8}{c}{Bad-3.0 Error Rates (\%)}  \\
	 &{EPE(px)}  &{$\geq 1$ px} &{$\geq 3$ px} &{EPE(px)}  &{$\geq 1$ px} &{$\geq 3$ px} &{EPE(px)}  &{$\geq 1$ px} &{$\geq 3$ px} &{EPE(px)}  &{$\geq 1$ px} &{$\geq 3$ px} \\
	%\hline \hline
	\Xhline{2\arrayrulewidth}
	W/O & 0.70 & 10.28 & 3.12  & 0.48   & 5.16  & 1.96  & 0.30  & \textbf{3.09} & 1.0563  & 0.59  & 7.48 & 2.25 \\
	%\hline
	\Xhline{2\arrayrulewidth}
	\cellcolor{myskyblue}SABF & \cellcolor{mygray}0.69 & \cellcolor{mygray} 9.75 & \cellcolor{mygray} 3.00  & \cellcolor{mygray}0.44 & \cellcolor{mygray}4.47 & \cellcolor{mygray}1.73  & \cellcolor{mygray}\textbf{0.28} & 3.16 & \cellcolor{mygray}\textbf{0.97}  & \cellcolor{mygray}0.56 & 7.51  & \cellcolor{mygray}2.23  \\
	\cellcolor{myskyblue} DFN & \cellcolor{mygray} \textbf{0.599} & \cellcolor{mygray}8.54 & \cellcolor{mygray}\textbf{2.791}  & \cellcolor{mygray}\textbf{0.39}  & \cellcolor{mygray}4.83 & \cellcolor{mygray}\textbf{1.69}  & \cellcolor{mygray}0.29  & 3.54 & \cellcolor{mygray}\textbf{1.0561}  & \cellcolor{mygray}0.55 & \cellcolor{mygray}6.81 & \cellcolor{mygray}\textbf{2.14}  \\
	\cellcolor{myskyblue}PAC & \cellcolor{mygray}0.603 & \cellcolor{mygray}8.73 & \cellcolor{mygray}2.96  & 0.52  & 5.78  & 1.98   & 0.35  & 4.36 & 1.47  & 0.73 & 11.87 & 2.99  \\
	\cellcolor{myskyblue}SGA & \cellcolor{mygray}0.607 & \cellcolor{mygray}\textbf{8.02} & \cellcolor{mygray}2.794 & \cellcolor{mygray}0.42 & \cellcolor{mygray}\textbf{4.34} & \cellcolor{mygray}1.71  &- &- &-  & \cellcolor{mygray}\textbf{0.53} & \cellcolor{mygray}\textbf{7.45} & 2.29  \\
	%\hline
	\Xhline{2\arrayrulewidth}
	\end{tabularx}}

\caption*{(b) Evaluation on VKT2 validation set of Scene06. No frames in this scene have been used during training.}
\label{tab:vkt2-val-scene06}

\vspace{-4pt}
\caption{Evaluation on Virtual KITTI 2 validation set. 
%The error metric $\geq$ 1 (or $3$) px shows the ratio of bad pixels with estimation error $\geq 1$ (or $3$) pixels or $\geq 5$\% of the true disparity. 
Ours are shown in the entries of filters (rows in skyblue) and backbones (columns) w.r.t. the baselines (row W/O). Our improved results are highlighted in gray, and the best ones are in bold. GANet contains the SGA filter, resulting in blank entries (-). 
%See texts for more details.
}
\label{tab:vkt2-val}
\end{table*}

==> experiments.tex <==
\subsection{Datasets}

Our networks are trained from scratch on Scene Flow \cite{mayer2016large}, then finetuned on Virtual KITTI 2 (VKT2) \cite{cabon2020virtual,gaidon2016virtual} or KITTI 2015 (KT15) \cite{menze2015object}. \textbf{Scene Flow} is a large scale synthetic dataset containing $35,454$ training and $4,370$ testing images with dense ground truth disparity maps.
%with dimensions $540 \times 960$. 
We exclude the pixels with disparities $d>192$ in training.
\textbf{Virtual KITTI 2 (VKT2)} is a synthetic clone of the real KITTI dataset. It contains 5 sequence \textit{clones} of {\myqcrfont Scene 01, 02, 06, 18} and {\myqcrfont 20}, and nine variants with diverse weather conditions (e.g. {\myqcrfont fog, rain}) or modified camera configurations (e.g. rotated by $15 \degree$, $30 \degree$). Since there is no designated validation set, we select (i) {\myqcrfont Scene06} (i.e., \textit{VKT2-Val-S6} with $2,700$ frames) and (ii) multiple blocks of consecutive frames from {\myqcrfont Scene 01, 02, 18, 20} (i.e., \textit{VKT2-Val-WoS6} with $2,620$ frames), and use the remaining $15,940$ images for training. The former scene remains unseen during training, while networks observe similar frames to the latter. We evaluate these settings separately.
\textbf{KITTI 2015 (KT15):} is a real dataset of street views.
% from a driving car. 
It contains $200$ training stereo image pairs with sparsely labeled disparity from LiDAR data. We divided the training data into a training set ($170$ images) and a validation set ($30$ images) for our experiments.



\noindent \textbf{Metrics.} \, %All algorithms are evaluated on the above validation sets. 
For KT15, we adopt the %\textit{D1-all} error
\textit{bad-3} error
(i.e., percentage of pixels with disparity error $>3$px or $\geq 5\%$ of the true disparity) counted over non-occluded (noc) or all pixels with ground truth. For VKT2, in addition to \textit{bad-3}, we also use the endpoint error (EPE) and \textit{bad-1} error ($\geq 1$px or $\geq 5\%$) over all pixels.
    

\begin{table*}[t]
\small
\centering
\scalebox{0.96}{
    %\begin{tabularx}{1.0\linewidth}{p{0.75cm} | XX XX XX XX}
    %\begin{tabularx}{1.0\linewidth}{@{} p{0.75cm} | YYY| YYY |YYY | YYY @{}}
    \begin{tabularx}{1.0\linewidth}{@{} ?{1pt} p{0.75cm} ?{1pt} YYY ?{1pt} YYY  ?{1pt}YYY ?{1pt} YYY ?{1pt} @{}}
    %\hline
    \Xhline{2\arrayrulewidth}
	\multirow{3}{0.8pt}{{\bf Filters}} & \multicolumn{3}{c ?{1pt} }{ \bf DispNetC} & \multicolumn{3}{c ?{1pt}  }{ \bf PSMNet}  & \multicolumn{3}{c ?{1pt}  }{ \bf GANet} & \multicolumn{3}{c ?{1pt}}{ \bf GCNet} \\
	\cline{2-13} % draw a horizontal line spanning only some of the table cells
	%&\multicolumn{8}{c}{Bad-3.0 Error Rates (\%)}  \\
	 &{EPE(px)}  &{$\geq 1$ px} &{$\geq 3$ px} &{EPE(px)}  &{$\geq 1$ px} &{$\geq 3$ px} &{EPE(px)}  &{$\geq 1$ px} &{$\geq 3$ px} &{EPE(px)}  &{$\geq 1$ px} &{$\geq 3$ px} \\
	%\hline \hline
	\Xhline{2\arrayrulewidth}
	\multicolumn{13}{ ?{1pt} c ?{1pt}  }{ \textit{Seen locations (i.e., Scene01, 02, 18 and 20) from VKT2 validation set \textbf{VKT2-Val-WoS6}}} \\
	\hline
	W/O & 0.68 & 11.54 & 3.72  &0.45   & 7.08  & 2.21  & \textbf{0.33}  & \textbf{5.34} & \textbf{1.70}  & 0.62  & 9.71 & 3.18 \\
	\hline
	%\Xhline{2\arrayrulewidth}
	\cellcolor{myskyblue}SABF & \cellcolor{mygray}0.65 & \cellcolor{mygray} 10.86 & \cellcolor{mygray} 3.48  & \cellcolor{mygray}\textbf{0.36} & \cellcolor{mygray}\textbf{5.92} & \cellcolor{mygray}\textbf{1.98}  & 0.34 & 5.50 & 1.76  & \cellcolor{mygray}0.60 & 9.89  & 3.19  \\
	\cellcolor{myskyblue} DFN & \cellcolor{mygray} \textbf{0.57} & \cellcolor{mygray}9.85 & \cellcolor{mygray}3.26  & \cellcolor{mygray}0.42  & \cellcolor{mygray}6.45 & \cellcolor{mygray}2.17  & 0.37  & 6.23 & 1.99  & \cellcolor{mygray}0.60 & \cellcolor{mygray}9.20 & \cellcolor{mygray}3.11  \\
	\cellcolor{myskyblue}PAC & \cellcolor{mygray}0.58 & \cellcolor{mygray}9.92 & \cellcolor{mygray}3.39  & 0.52  & 7.81  & 2.61   & 0.40  & 7.01 & 2.20  & 0.75 & 12.98 & 4.02  \\
	\cellcolor{myskyblue}SGA & \cellcolor{mygray}\textbf{0.57} & \cellcolor{mygray}\textbf{9.37} & \cellcolor{mygray}\textbf{3.21} & \cellcolor{mygray}0.40 & \cellcolor{mygray}6.08 & \cellcolor{mygray}2.14  &- &- &-  & \cellcolor{mygray}\textbf{0.55} & \cellcolor{mygray}\textbf{9.24} & \cellcolor{mygray}\textbf{2.98}  \\
	%\hline
	\Xhline{2\arrayrulewidth}
	
    \multicolumn{13}{ ?{1pt} c ?{1pt}  }{ \textit{Totally unseen location (i.e., Scene06) from VKT2 validation set \textbf{VKT2-Val-S6}}} \\
	\hline
	%\Xhline{2\arrayrulewidth}
	W/O & 0.70 & 10.28 & 3.12  & 0.48   & 5.16  & 1.96  & 0.30  & \textbf{3.09} & 1.0563  & 0.59  & 7.48 & 2.25 \\
	\hline
	%\Xhline{2\arrayrulewidth}
	\cellcolor{myskyblue}SABF & \cellcolor{mygray}0.69 & \cellcolor{mygray} 9.75 & \cellcolor{mygray} 3.00  & \cellcolor{mygray}0.44 & \cellcolor{mygray}4.47 & \cellcolor{mygray}1.73  & \cellcolor{mygray}\textbf{0.28} & 3.16 & \cellcolor{mygray}\textbf{0.97}  & \cellcolor{mygray}0.56 & 7.51  & \cellcolor{mygray}2.23  \\
	\cellcolor{myskyblue} DFN & \cellcolor{mygray} \textbf{0.599} & \cellcolor{mygray}8.54 & \cellcolor{mygray}\textbf{2.791}  & \cellcolor{mygray}\textbf{0.39}  & \cellcolor{mygray}4.83 & \cellcolor{mygray}\textbf{1.69}  & \cellcolor{mygray}0.29  & 3.54 & \cellcolor{mygray} 1.0561  & \cellcolor{mygray}0.55 & \cellcolor{mygray}6.81 & \cellcolor{mygray}\textbf{2.14}  \\
	\cellcolor{myskyblue}PAC & \cellcolor{mygray}0.603 & \cellcolor{mygray}8.73 & \cellcolor{mygray}2.96  & 0.52  & 5.78  & 1.98   & 0.35  & 4.36 & 1.47  & 0.73 & 11.87 & 2.99  \\
	\cellcolor{myskyblue}SGA & \cellcolor{mygray}0.607 & \cellcolor{mygray}\textbf{8.02} & \cellcolor{mygray}2.794 & \cellcolor{mygray}0.42 & \cellcolor{mygray}\textbf{4.34} & \cellcolor{mygray}1.71  &- &- &-  & \cellcolor{mygray}\textbf{0.53} & \cellcolor{mygray}\textbf{7.45} & 2.29  \\
	%\hline
	\Xhline{2\arrayrulewidth}
	\end{tabularx}}
\vspace{-4pt}
\caption{Evaluation on VKT2 validation sets of VKT2-Val-WoS6 and VKT2-Val-S6. 
%The error metric $\geq$ 1 (or $3$) px shows the ratio of bad pixels with estimation error $\geq 1$ (or $3$) pixels or $\geq 5$\% of the true disparity. 
Results are shown in the entries of filters (rows in skyblue) and backbones (columns) w.r.t. the baselines (rows W/O). Our improved results are highlighted in gray, and the best ones are in bold. GANet already contains SGA, resulting in blank entries ``-''.
}
\label{tab:vkt2-val}
\end{table*}

\input{vkt2_plot}


\subsection{Implementation Details}

\vspace{3pt} \noindent \textbf{Architecture details.} \, Our models are implemented with PyTorch. Each convolution layer is followed by batch normalization (BN) and ReLU unless otherwise specified. We use the official code of PSMNet and GANet, and implement DispNetC (no PyTorch version) and GCNet (no official code). Our implementations achieve similar or better results on the  KT15  benchmark, i.e., bad-3 errors $4.48\%$ (all) and $3.85\%$ (noc) versus the authors' $4.34\%$ (all) and $4.05\%$ (noc) for DispNetC, and $2.38\%$ (all) and $2.07\%$ (noc) versus the authors' $2.87\%$ (all) and $2.61\%$ (noc) for GCNet.
% D1-all error  of  2.76%  (versus  2.87%  as  reported by GCNet).
%There is no BN layer after several convolution layers which output disparity maps in DispNetC and hence in our DispNetC variant. %
We use $\sigma_s=0.7$ and $\sigma_r=0.1$ in Eq. \ref{eq:ebf-filter} for SABF. We investigate how the filter window $s$ and dilation rate $r$ affect the filtering output, and find that $s=5$ with $r=2$ achieve a good balance in accuracy, space requirements and runtime. Please see the supplementary material for ablation studies.


\vspace{3pt} \noindent \textbf{Training details.} \, The SABF embedding network is pre-trained on Cityscapes \cite{cordts2016cityscapes}. For data augmentation we randomly crop $256 \times 512$ image patches and do channel-wise standardization by subtracting the mean and dividing by the standard deviation. % per channel. 
For fair comparison, we follow the baselines and set the maximum disparity to $D=192$. We use the official pre-trained models on Scene Flow for GANet and PSMNet, and train DispNetC and GCNet on Scene Flow from scratch for $10$ epochs with a learning rate (lr) of $0.001$. Training is optimized with Adam ($\beta_1 = 0.9$, $\beta_2 = 0.999$), except for GCNet which uses RMSprop ($\alpha=0.9$).  For KT15, our models and baselines are finetuned for 600 epochs (with lr$=0.001$ for the first $300$ epochs and lr$=0.0001$ for the next $300$ epochs). For VKT2, we finetune all algorithms for $20$ epochs, with lr $=0.001$ at first, then divided by 10 at epoch 5 and epoch 18.

% solve: Losing the vertical line on my table when using multicolumn 
%Answer: change \multicolumn{11}{l}{...} to \multicolumn{11}{l|}{...} 



% \subsection{Ablation Study}
%  We perform ablation studies to investigate how the filter window $s$ and the dilation rate $r$ can affect the filtering output and disparity estimation. Out of a large number of possible combinations, %we cannot take the ablation study on each of them. 
%  we show \textit{SABF+DispNetC} as a representative. %due to its computational efficiency. 
%  As listed in Table \ref{tab:filter_size_kt15-val30}, we find $s=5$ with $r=2$ achieves a good balance in accuracy, space and runtime. 
%  %The 500-run averaged memory and runtime in GPUs are measured when we test a $384 \times 1280$ stereo pair, and the \textit{bad-3} (noc,all) errors are evaluated on the KITTI 2015 validation set. 
%  Please note that a $5 \times 5$ filter (with dilation rate $2$) covers $9 \times 9$ regions in the cost feature space, which is equivalent to $33 \times 33$ regions in the RGB image space, due to the cost volume being a quarter of the size of the input images. In the following experiments, we keep using $s = 5$ with $r = 2$ for our different architectures.
 
 % Leave a note here: how it is obtained: s = 5, r = 2, (s-1) * r * (img_size / cost_size) + 1 = 33;
 
\subsection{Quantitative Results}
All results are on the \textit{validation sets} since we could not submit all combinations to the benchmarks. Due to page limits, qualitative results are available in the supplementary material.


\vspace{3pt} \noindent \textbf{Virtual KITTI 2 Evaluation.} \,We finetune our models (the pre-trained backbones on Scene Flow after integrating the filters) on the VKT2 dataset. (\textit{EPE}, \textit{bad-1} and \textit{bad-3}) on the \textit{VKT2-Val-WoS6} and \textit{VKT2-Val-S6} validation sets are listed in Table \ref{tab:vkt2-val}. In most cases, our models (rows in skyblue) achieve higher accuracy than the baselines (row W/O). The exception is standard GANet which performs well since it always includes SGA and LGA for global and local matching volume aggregation. Fig. \ref{fig:vkt2-val-s6} plots EPE errors on \textit{individual} categories of \textit{VKT2-Val-S6}. %Recall that DispNetC belongs to 2D CNNs and the others belong to 3D CNNs. 
SABF, DFN and SGA  boost 2D and 3D CNNs, while PAC improves 2D CNNs, but not 3D CNNs. When moving from familiar  (\textit{VKT2-Val-WoS6}) to unseen (\textit{VKT2-Val-S6}) validation scenes, DFN achieves better adaptation than SGA, and the SABF and DFN variants outperform standard GANet.



%\subsection{KITTI 2015 Evaluation}
\begin{table}[b]
\small
\centering
\scalebox{0.95}{
    %\begin{tabularx}{1.0\linewidth}{p{0.75cm} | XX XX XX XX}
    %\begin{tabularx}{1.0\linewidth}{@{} p{0.75cm} | YY| YY| YY| YY @{}}
    %note: ?{1pt} is used to draw a thick vertical line;
    \begin{tabularx}{1.0\linewidth}{@{} ?{1pt} p{0.75cm}?{1pt}  YY ?{1pt}  YY ?{1pt} YY ?{1pt} YY ?{1pt} @{}}
    %\hline
    \Xhline{2\arrayrulewidth}
	\multirow{3}{0.8pt}{{\bf Filters}} & \multicolumn{2}{c ?{1pt}}{\bf DispNetC} & \multicolumn{2}{c?{1pt}}{ \bf PSMNet}  & \multicolumn{2}{c?{1pt}}{ \bf GANet} & \multicolumn{2}{c?{1pt}}{ \bf GCNet} \\
	\cline{2-9} % draw a horizontal line spanning only some of the table cells
	%&\multicolumn{8}{c}{Bad-3.0 Error Rates (\%)}  \\
	%\cline{2-9} % draw a horizontal line spanning only some of the table cells
	 &{noc}  &{all} &{noc}  &{all} &{noc}  &{all} &{noc}  &{all} \\
	%\hline \hline
	\Xhline{2\arrayrulewidth}
	W/O & 2.59 & 3.02 & 1.46  & 1.60  & \textbf{0.97}  & \textbf{1.10}   & 2.06  & 2.64  \\
	\Xhline{2\arrayrulewidth}
	\cellcolor{myskyblue} SABF & \cellcolor{mygray}2.26 & \cellcolor{mygray}2.63 & \cellcolor{mygray}1.28  & \cellcolor{mygray}1.40  & 1.07 & 1.17   & \cellcolor{mygray}1.76  & \cellcolor{mygray} 2.10  \\
	\cellcolor{myskyblue} DFN & \cellcolor{mygray} 2.37 & \cellcolor{mygray} 2.78  & \cellcolor{mygray} 1.23  & \cellcolor{mygray} 1.34  & 0.99  & 1.11   & \cellcolor{mygray} 1.70  & \cellcolor{mygray} 2.08  \\
	\cellcolor{myskyblue} PAC & \cellcolor{mygray} 2.38  & \cellcolor{mygray} 2.72  & \cellcolor{mygray} 1.29  & \cellcolor{mygray} 1.48  & 1.13  & 1.23   & \cellcolor{mygray} 1.71  & \cellcolor{mygray} 2.03  \\
	\cellcolor{myskyblue} SGA & \cellcolor{mygray}\textbf{1.90}  & \cellcolor{mygray}\textbf{2.18}  & \cellcolor{mygray}\textbf{1.17}  & \cellcolor{mygray}\textbf{1.32}  & - & -  & \cellcolor{mygray}\textbf{1.69}   & \cellcolor{mygray}\textbf{1.91}  \\
	\Xhline{2\arrayrulewidth}
	\end{tabularx}}
\vspace{-4pt}
\caption{KITTI 2015 bad-3 validation results. Improved results are highlighted in gray, and best ones are in bold. GANet contains SGA, resulting in blank entries ``-''.}
\label{tab:kt15-val30}
\end{table}

 
\vspace{3pt} \noindent \textbf{KITTI 2015 Evaluation.} \,The results on KT15 are shown in Table \ref{tab:kt15-val30}. Our networks obtain improved accuracy for all the backbones except for GANet. All the filters boost the backbones due to leveraging image context as guidance, and SGA achieves the highest accuracy among them.  

%See methods effectiveness comparison on KITTI 2015 val-30 dataset in Table \ref{tab:model-effect-kt15-val30}.



% move it to the supplement
%\subsection{Complexity and Runtime} 
% See methods effectiveness comparison on KITTI 2015 val-30 dataset in Table \ref{tab:model-effect-kt15-val30}.
